Hyperbolic Graph Convolutional Neural Networks

Graph convolutional neural networks (GCNs) embed nodes in a graph into Euclidean space, which has been shown to incur a large distortion when embedding real-world graphs with scale-free or hierarchical structure. Hyperbolic geometry offers an exciting alternative, as it enables embeddings with much smaller distortion. However, extending GCNs to hyperbolic geometry presents several unique challenges because it is not clear how to define neural network operations, such as feature transformation and aggregation, in hyperbolic space. Furthermore, since input features are often Euclidean, it is unclear how to transform the features into hyperbolic embeddings with the right amount of curvature. Here we propose Hyperbolic Graph Convolutional Neural Network (HGCN), the first inductive hyperbolic GCN that leverages both the expressiveness of GCNs and hyperbolic geometry to learn inductive node representations for hierarchical and scale-free graphs. We derive GCN operations in the hyperboloid model of hyperbolic space and map Euclidean input features to embeddings in hyperbolic spaces with different trainable curvature at each layer. Experiments demonstrate that HGCN learns embeddings that preserve hierarchical structure, and leads to improved performance when compared to Euclidean analogs, even with very low dimensional embeddings: compared to state-of-the-art GCNs, HGCN achieves an error reduction of up to 63.1% in ROC AUC for link prediction and of up to 47.5% in F1 score for node classification, also improving state-of-the art on the Pubmed dataset.

==> ablation.tex <==
\begin{comment}
\scriptsize
\begin{wraptable}{r}{0.4\textwidth}
%\begin{table}{}
%\resizebox{\textwidth}{!}{ \renewcommand{\arraystretch}{1.0}
  %\vspace{-25pt}
  %\vspace{-40pt}
  \begin{center}
  \begin{tabular}{@{}clccc@{}}
%\cmidrule[\heavyrulewidth]{2-6}
\hline
\multirow{1}{*}{\vspace*{8pt}\textbf{Method}}&\multicolumn{1}{c}{\textsc{Disease}} & \multicolumn{1}{c}{\textsc{Airport}}
\\ 
%\cmidrule{1-4}
\hline
\textsc{\HGCN} & 78.4 $\pm$ 0.3 & 91.8 $\pm$ 0.3 \\
\textsc{\HGCN-Att}_\mathbf{o} & 80.9 \pm 0.4 & 92.3 $\pm$ 0.3 \\
\textsc{\HGCN-Att} & 82.0 $\pm$ 0.2 & 92.5 $\pm$ 0.2 \\
%\textsc{\HGCN-Lorentz} &   &   \\
\textsc{\HGCN-C} & 89.1 $\pm$ 0.2 & 94.9 $\pm$ 0.3 \\
\textsc{\HGCN-Att-C} & \textbf{90.8} $\pm$ 0.3 & \textbf{96.4} $\pm$ 0.1 \\
% GNN
%& \textsc{HGCN-H}  &   &  &   &  &    &  & &  & 92.4  & 86.7\\	  
%& \textsc{HGCN-Max}  &   &  &   &  &     &  \\
%& \textsc{HGCN-Att} & 83.9  &  &   &  &   & & 85.5  & 60.9 & 94.6 & 90.5\\
%& \textsc{HGCN-C}  &  94.1 &  &   &  & & & 83.0  & 62.8 & & 91.9  & \\	  
%\cmidrule{1-4}	  
\hline
%\cmidrule[\heavyrulewidth]{2-4}
\end{tabular}
  \end{center}
  %\vspace{-10pt}
  \caption{ROC AUC for link prediction on \textsc{Airport} and \textsc{Disease} datasets.}
  %}
\label{tab:ablations}
%\end{table}
%\vspace{-5pt}
\end{wraptable}
%
\normalsize
% * indicate numbers reported in corresponding papers.}

%\resizebox{\textwidth}{!}{ 
%\renewcommand{\arraystretch}{1.0}
\end{comment}

==> figs/poincare.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
 %\vspace{-15pt}
  \begin{center}
  \includegraphics[width=\linewidth]{figs/curvature_geodesics.pdf}
\caption{Left: Poincar\'{e} disk geodesic lines connecting $\mathbf{x}$ and $\mathbf{y}$. 
Right: Hyperbolic distance vs curvature. As the radius $K$ increases (curvature $-1/K^2$ decreases), hyperbolic distances increase and the geodesics lines get closer to the zero.}
  \label{fig:poincare_geodesics}
  \end{center}
  %\vspace{-20pt}
\end{wrapfigure}


==> instructions.tex <==
\section{Submission of papers to NeurIPS 2019}


NeurIPS requires electronic submissions.  The electronic submission site is
\begin{center}
  \url{https://cmt.research.microsoft.com/NeurIPS2019/}
\end{center}

Please read the instructions below carefully and follow them faithfully.
\subsection{Abstract}
  The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on
  both the left- and right-hand margins. Use 10~point type, with a vertical
  spacing (leading) of 11~points.  The word \textbf{Abstract} must be centered,
  bold, and in point size 12. Two line spaces precede the abstract. The abstract
  must be limited to one paragraph.

\subsection{Style}

Papers to be submitted to NeurIPS 2019 must be prepared according to the
instructions presented here. Papers may only be up to eight pages long,
including figures. Additional pages \emph{containing only acknowledgments and/or
  cited references} are allowed. Papers that exceed eight pages of content
(ignoring references) will not be reviewed, or in any other way considered for
presentation at the conference.

The margins in 2019 are the same as since 2007, which allow for $\sim$$15\%$
more words in the paper compared to earlier years.

Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.

\subsection{Retrieval of style files}

The style files for NeurIPS and other conference information are available on
the World Wide Web at
\begin{center}
  \url{http://www.neurips.cc/}
\end{center}
The file \verb+neurips_2019.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.

The only supported style file for NeurIPS 2019 is \verb+neurips_2019.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}

The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.

\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS.

At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.

The file \verb+neurips_2019.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.

The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.

The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.

For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.

Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}

All headings should be lower case (except for first word and proper nouns),
flush left, and bold.

First-level headings should be in 12-point type.

\subsection{Headings: second level}

Second-level headings should be in 10-point type.

\subsubsection{Headings: third level}

Third-level headings should be in 10-point type.

\paragraph{Paragraphs}

There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone.

\subsection{Citations within the text}

The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.

The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}

If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2019+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}

If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2019}
\end{verbatim}

As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous.''

\subsection{Footnotes}

Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).

Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}

\subsection{Figures}

\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}

All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.

You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.

\subsection{Tables}

All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.

Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.

Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.

\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\section{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PDF files}

Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''

Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.

\begin{itemize}

\item You should directly generate PDF files using \verb+pdflatex+.

\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.

\item The IEEE has recommendations for generating PDF files whose fonts are also
  acceptable for NeurIPS. Please see
  \url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}

\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.

\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.

\end{itemize}

If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.

\subsection{Margins in \LaTeX{}}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})

A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.

\subsubsection*{Acknowledgments}

Use unnumbered third level headings for the acknowledgments. All acknowledgments
go at the end of the paper. Do not include acknowledgments in the anonymized
submission, only in the final paper.

\section*{References}

References follow the acknowledgments. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references. {\bf Remember that you can use more than eight
  pages as long as the additional pages contain \emph{only} cited references.}
\medskip

\small

[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.

[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.

[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.

==> table_std.tex <==
\begin{table}[t]	
\resizebox{\textwidth}{!}{ \renewcommand{\arraystretch}{1.0}
\centering
\begin{tabular}{@{}clcccccccccccc@{}}\cmidrule[\heavyrulewidth]{2-14}
& %\multirow{2}{*}{\vspace*{8pt}\textbf{Dataset and Hyperbolicity}}
\textbf{Dataset} &\multicolumn{2}{c}{\textsc{Disease}} & \multicolumn{2}{c}{\textsc{Disease-M}} & \multicolumn{2}{c}{\textsc{\textsc{Human PPI}}} & \multicolumn{2}{c}{\textsc{Airport}}  &  \multicolumn{2}{c}{\textsc{PubMed}} & \multicolumn{2}{c}{\textsc{Cora}} \\
& \textbf{Hyperbolicity $\delta$} & \multicolumn{2}{c}{$\delta=0$} & \multicolumn{2}{c}{$\delta=0$} &\multicolumn{2}{c}{$\delta=1$} &\multicolumn{2}{c}{$\delta=1$} & \multicolumn{2}{c}{$\delta=3.5$} & \multicolumn{2}{c}{$\delta=11$}
\\\cmidrule{3-14}
& \textbf{Method} & {\textsc{LP}} & {\textsc{NC}} & {\textsc{LP}} & {\text{NC}} & {\textsc{LP}} & {\text{NC}} & {\textsc{LP}} & {\text{NC}} & {\textsc{LP}} & {\text{NC}} & {\textsc{LP}} & {\text{NC}}
\\ \cmidrule{2-14}
\multirow{4}{*}{\rotatebox{90}{\hspace*{-6pt} Shallow}} 
& \textsc{Euclidean} & 59.8 $\pm$ 2.0 & 32.5 $\pm$ 1.1 & -  & -  & -  & - & 92.0 $\pm$ 0.0& 60.9 $\pm$ 3.4 & 83.3 $\pm$ 0.1 & 48.2 $\pm$ 0.7 & 82.5 $\pm$ 0.3 & 23.8 $\pm$ 0.7\\ 
& \textsc{Poincare} \cite{nickel2017poincare} & 63.5 $\pm$ 0.6 &  45.5 $\pm$ 3.3 & -  &  -  & - & - & 94.5 $\pm$ 0.0& 70.2 $\pm$ 0.1 & 87.5 $\pm$ 0.1 & 68.5 $\pm$ 0.3 & 87.6 $\pm$ 0.2 & 22.0 $\pm$ 1.5  \\     
& \textsc{Euclidean-Mixed} &  49.6 $\pm$ 1.1 & 35.2 $\pm$ 3.4 & -  &  - &  - & - & 91.5 $\pm$ 0.1 &68.3 $\pm$ 2.3 & 86.0 $\pm$ 1.3 & 63.0 $\pm$ 0.3& 84.4 $\pm$ 0.2 & 46.1 $\pm$ 0.4   \\  
& \textsc{Poincare-Mixed} & 55.1 $\pm$ 1.3 &  56.9 $\pm$ 1.5 & -  &  -  & - & - & 93.3 $\pm$ 0.0& 69.6 $\pm$ 0.1 & 83.8 $\pm$ 0.3 & 73.9 $\pm$ 0.2& 85.6 $\pm$ 0.5 & 45.9 $\pm$ 0.3 \\  
\cmidrule{2-14}
\multirow{2}{*}{\rotatebox{90}{NN}}        
& \textsc{MLP} & 72.6 $\pm$ 0.6 & 15.2 $\pm$ 4.4 & 55.3 $\pm$ 4.9   &   & 67.8  & 55.3& 89.8 $\pm$ 0.5 & 68.6 $\pm$ 0.6 & 84.1 $\pm$ 0.9 & 72.4 $\pm$ 0.2 & 83.1 $\pm$ 0.5 & 51.5 $\pm$ 1.0 \\ 
% GNN
& \textsc{HNN\cite{ganea2018hyperbolicNN}} & 75.1 $\pm$ 0.3 & & & 57.4  & & & 90.8 $\pm$ 0.2 & 80.5 $\pm$ 0.5 & 94.9 $\pm$ 0.1 & 69.8 $\pm$ 0.4 & 89.0 $\pm$ 0.1 & 54.6 $\pm$ 0.4\\
\cmidrule{2-14}
\multirow{4}{*}{\rotatebox{90}{GNN}}
& \textsc{GCN}\cite{kipf2016semi} & 64.7 $\pm 0.5$ &  69.7 $\pm$ 0.4 &  66.0 $\pm$ 0.8  &  57.4 $\pm$ 3.4 & 77.0 $\pm$ 0.5  & 69.7 $\pm$ 0.3 & 89.3 $\pm$ 0.4 & 81.4 $\pm$ 0.6 & 91.1 $\pm$ 0.5 & 78.1 $\pm$ 0.2 & 90.4 $\pm$ 0.2 & 81.3 $\pm$ 0.3 \\ 
& \textsc{GAT} \cite{velickovic2017graph} & 69.8 $\pm 0.3$  & 70.4 $\pm$ 0.4 & 69.5 $\pm$ 0.4  &  62.5 $\pm$ 0.7 & 76.8 $\pm$ 0.4 & & 90.5 $\pm$ 0.3 & 81.5 $\pm$ 0.3 & 91.2 $\pm$ 0.1 & $\ 79.0 \pm$ 0.3* & \textbf{93.7 $\pm$ 0.1} & \ \textbf{83.0 $\pm$ 0.7}*\\ 
& \textsc{GraphSAGE} \cite{hamilton2017inductive} & 65.9 $\pm$ 0.3  &  69.1 $\pm$ 0.6 &  67.4 $\pm$ 0.5 & 59.3 $\pm$ 0.4 & 78.1 $\pm$ 0.6 & & 90.4 $\pm$ 0.5 & 82.1 $\pm$ 0.5 & 86.2 $\pm$ 1.0 & 77.4 $\pm$ 2.2 & 85.5 $\pm$ 0.6 & 77.9 $\pm$ 2.4  \\ 
%& \textsc{JKG} &   &  	 &   &   &  &  \\ 
& \textsc{SGC} \cite{wu2019simplifying} & 65.1 $\pm$ 0.2  &  69.5 $\pm$ 0.2	 & 66.2 $\pm$ 0.2 &  57.9 $\pm$ 0.3 & 76.1 $\pm$ 0.2 &  & 89.8 $\pm$ 0.3 & 80.6 $\pm$ 0.1 & 94.1 $\pm$ 0.0 &  78.9 $\pm$ 0.0 & 91.5 $\pm$ 0.1 & 81.0 $\pm$ $0.1$ \\ 
\cmidrule{2-14}
\multirow{3}{*}{\rotatebox{90}{Ours}} 
%& \textsc{\name} & $\mathbf{90.8}$ $\pm$ 0.3  & 74.5 $\pm$ 0.9 &  76.6 $\pm$ 3.1 & 71.8 $\pm$ 0.8 & & & 84.8  & 59.0 & 94.4 & 87.6 & \textbf{96.3 $\pm$ 0.0} & \textbf{80.3 $\pm$ 0.3} & 92.9 $\pm$ 0.1 & 79.9 $\pm$ 0.2 \\	
& \textsc{\name} & $\mathbf{90.8}$ $\pm$ 0.3  & 74.5 $\pm$ 0.9 &  $\mathbf{78.1}$ $\pm$ 0.4 & $\mathbf{74.5}$ $\pm$ 0.5 & $\mathbf{84.5}$ $\pm$ 0.4 & 79.1 $\pm$ 0.3 & $\mathbf{96.4}$ $\pm$ 0.1 & $\mathbf{90.6}$ $\pm$ 0.2 & \textbf{96.3 $\pm$ 0.0} & \textbf{80.3 $\pm$ 0.3} & 92.9 $\pm$ 0.1 & 79.9 $\pm$ 0.2 \\	 % with -att-C
%& \textsc{HGCN-H}  &   &  &   &  &    &  & &  & 92.4  & 86.7\\	  
%& \textsc{HGCN-Max}  &   &  &   &  &     &  \\
%& \textsc{HGCN-Att} & 83.9  &  &   &  &   & & 85.5  & 60.9 & 94.6 & 90.5\\
%& \textsc{HGCN-C}  &  94.1 &  &   &  & & & 83.0  & 62.8 & & 91.9   \\	  
\cmidrule{2-14}
& \textsc{($\%$) Gain}  & +20.91\%  &  & +15.88\%  & +25.63\% & +8.19\% &  & +7\% & +10.35\% & +1.45\% & +1.65\% & -0.85\% & -3.73\% \\	  
\cmidrule[\heavyrulewidth]{2-14}



\end{tabular}}
\caption{ROC AUC for Link Prediction (LP) and F1 score for Node Classification (NC) tasks. For inductive datasets, we only evaluate inductive methods since shallow methods cannot generalize to unseen nodes/graphs. We report graph hyperbolicity values $\delta$ (lower is more hyperbolic).}
% * indicate numbers reported in corresponding papers.}
\label{tab:results_appendix}
\end{table}
